Breaking Blockchain Rationality with Out-of-Band Collusion

Blockchain systems often rely on rationality assumptions for their security, expecting that nodes are motivated to maximize their profits. These systems thus design their protocols to incentivize nodes to execute the honest protocol but fail to consider out-of-band collusion. Existing works analyzing rationality assumptions are limited in their scope, either by focusing on a specific protocol or relying on non-existing financial instruments. We propose a general rational attack on rationality by leveraging an external channel that incentivizes nodes to collude against the honest protocol. Our approach involves an attacker creating an out-of-band bribery smart contract to motivate nodes to double-spend their transactions in exchange for shares in the attacker's profits. We provide a game theory model to prove that any rational node is incentivized to follow the malicious protocol. We discuss our approach to attacking the Bitcoin and Ethereum blockchains, demonstrating that irrational behavior can be rational in real-world blockchain systems when analyzing rationality in a larger ecosystem. We conclude that rational assumptions only appear to make the system more secure and offer a false sense of security under the flawed analysis.

==> Makefile <==
.PHONY: FORCE lenny all clean distclean

FILE=main

all: $(FILE).pdf

%.pdf: %.tex FORCE
	latexmk -pdf $<

fast:
	pdflatex -shell-escape $(FILE)

link:
	rm -f *.bib
	for lib in comp fault net os priv sec soc theory; do \
		ln -s ../$$lib.bib $$lib.bib ; \
	done

clean:
	for ext in aux log toc lof lot lol dlog bbl \
		nav snm fls vrb blg out tpt fdb_latexmk; \
	do \
		$(RM) $(FILE).$$ext ; \
	done
	$(RM) *.aux *.bak *~

distclean: clean
	$(RM) $(FILE).pdf
	$(RM) $(FILE).ps
	$(RM) $(FILE).dvi
	$(RM) *.d


==> content/4-analysis-new.tex <==
\section{Game Theoretic Analysis}\label{sec:gametheory}
In this section, 
we formalize the behavior of the \cns of {\Sys}
first without the presence of any external factors 
and then with the presence of the \bsc on \Sprime.
%first in the absence and then in the presence of the \smartContract. 
% LHM: without the absence of \smartContract imo is clearer that we only
% care about \Sys; there exists no external factors that could induce this coalition.
%
We use the notion of Evolutionarily Stable \NE to model the dynamics of \Sys when a fraction of the \cns adapt a malicious strategy. 
%
 Evolutionarily Stable strategy (ESS) is an effective and conventional approach for analyzing systems in which players converge to a stable
equilibrium after a period of interactions \cite{jiang2013joint}.
%

We formally define Evolutionarily Stable \NE in subsection \ref{subsec:ESS}; And in subsections  \ref{subsec:game0} and \ref{subsec:game1} we demonstrate how the existence of \bsc changes the situation of $\Ph$ from a stable equilibrium to an unstable one.
%
 Moreover, in subsection \ref{subsec:game1} we prove that in the presence of a \bsc, following the \bsc's attack is the only ESS of the game.
%
This implies that following the \bsc is the only equilibrium that survives in the system, and therefore our proposed attack is successful.

\subsection{Evolutionarily stable strategies (ESS)}\label{subsec:ESS}
The evolutionarily stable strategies (ESS) or evolutionary equilibrium is a refinement of Nash equilibrium. A strategy is ESS if deviating a relatively small portion of the population from that strategy does not incentives others to deviate too \cite{maschler2020game,han2012game}.
%
We first define ESS in a symmetric two-player game in which the player $1$ interacts with a member of a population and wants to find the strategy that yields the best reward on average.
%
Later, in subsection \ref{subsec:game0} we adapt the ESS definition to our setting where there are arbitrary number of nodes.

\begin{definition}
Let $\util(s, s')$ denote the payoff of player $1$ when player $1$ chooses strategy $s$ and player $2$ chooses strategy $s'$. Strategy $s$ is called evolutionarily stable if, for each strategy $s'\neq s$ there is $\hat{\epsilon} > 0$ such that the following holds:
$$\epsilon \util(s, s') + (1-\epsilon) \util(s,s) > \epsilon \util(s', s') + (1-\epsilon) \util(s', s) $$
for all $\epsilon \in (0,\hat{\epsilon})$ \cite{han2012game,maschler2020game}.
\end{definition} 
%

This definition can be interpreted as follow: when player $1$ encounters a population in which people play strategy $s$ with probability $1-\epsilon$ and strategy $s'$ with probability $\epsilon$, on average, player $1$ strictly benefits from playing $s$, as long as $\epsilon < \epsilon'$. 
%
Therefore every single player, when encountering this population, chooses $s$; as more players adopt $s$, $\epsilon$ (the percentage of the population that play $s'$) reduces, and playing $s$ becomes more beneficial.
%
So $s$ acts as the stable point of the system, that if a small portion of the system deviate from it, others still prefer to follow it, and the system always returns to the state where everybody plays $s$.
%
In fact, ESS captures the dynamics of a population instead of a single game between two parties.
%

The following theorem suggests a practical way to find ESS.
\begin{theorem}\label{theorem:ESS}
Strategy $s^{*}$ is evolutionarily stable if and only if for each $s' \neq s^{*}$ one of the following two conditions obtains:

\begin{itemize}
    \item $\util(s^{*},s^{*}) > \util(s',s^{*})$
     \item $\util(s^{*},s^{*}) = \util(s',s^{*})$  and  $\util(s^{*},s') > \util(s',s')$. 
\end{itemize}
     \cite{han2012game,maschler2020game}
     \zhq{Is this right place to put the citations? how about put inside "The following theorem suggests a practical way to find ESS."?}
\end{theorem}
There are three reasons why we specifically use the notion of ESS to analyze the behavior of nodes in Blockchains. First, we will see later in the \ref{subsec:game0} that our games have multiple {\NE}s, and we need to define some criteria (for instance \textit{stability}) to rule out the equilibriums that are less likely to be widely adopted in the \Sys. The second and more important reason is that \NE is a static and rather weak notion because it only guarantees that a single user would not benefit by deviation. However, ESS guarantees that even if a fraction of the \cns deviate (irrationally), the rest still prefer to follow the ESS. \cite{tembine2009evolutionary,jiang2013joint}.
%
Moreover, the former research on distributed systems widely adopts 
the concept of ESS to determine the stability or robustness of protocols \cite{tembine2009evolutionary,jiang2013joint,jiang2014equivalence}.
%
Now we are ready to model the system \Sys as a game and find its ESSs. 

\subsection{Game 0: Without Collusion}\label{subsec:game0}
 We define the game $\Gamma_0$ where its players are the \Sys's nodes $\N = \{1,2,\dots,N\}$. 
 %
 Each player has two strategies, following the protocol $\Ph$ or $\Pm$. Consider an arbitrary player $i$; $i$'s payoff is a function of its and other players' strategies.
 %
 We define $\Vh := \sum_{j \in \Nh} \vi$, the sum of \power of players who follow $\Ph$.
 %
 And similarly, we define $\Vm := \sum_{j \in \Nm} \vi$, the sum of \power of players who follow the malicious protocol. Note that we have normalized the \power therefore $\Vh + \Vm =1$
 %
  
  When $\Vh \geq \threshold$ i.e., $\Ph$ is the working protocol in \Sys, if $i \in \Nh$, $i$ obtain reward $\Rhi$, and if $i \in \Nm$ it obtains payoff $\Rdi$ which is certainly less than $\Rhi$ and can be even negative.
  %

 When $\Vh < \threshold$, since $t>\frac12$, $\Vm$ might or might not be larger than $\threshold$. If $\Vm$ is greater than $\threshold$, $\Pm$ is working in the \Sys, and any player $i \in \Nm$ gets reward $\Rmi$, whereas any player $i \in \Nh$ get payoff $\Rdpi < \Rmi$ (possibly negative). 
 %
 However, if $\Vh < \threshold$ and $\Vm$ is not greater than the $\threshold$, neither $\Ph$ nor $\Pm$ are working correctly, and the payoffs can be arbitrary. 
 %
 Nevertheless, in this subsection, we consider that whenever $\Vh < \threshold$, nodes get the same payoff as if $\Pm$ is working. We will see later that this simplifying assumption doesn't impact our argument at all. Because in this subsection we want to argue that $\Ph$ is a stable \NE and this simplifying assumption only changes the game in favor of $\Pm$.
%

In the game, $\Gamma_0$ where no factor outside of \Sys exists, both $\Ph$ and $\Pm$ are \NE and in the following, we show that $\Ph$ is a stable \NE as well. However, in subsection \ref{} we will see that in the presence of the \bsc, even though $\Ph$ is still a \NE but it is not a stable \NE anymore.

Table \ref{tabular:game0} demonstrates the payoff of an arbitrary player $i$ for different values of $\Vh$.
%
 From the player $i$'s perspective, it doesn't matter that $\Vh$ is determined by the decision of multiple nodes or a single node. The only thing that affects $i$'s payoff is the value of $\Vh$.
%
 Therefore we can consider $\Vh$ as the strategy of an imaginary/virtual player and analyze the behavior of $i$ when encountering this virtual player.
%

 Let's review the concept of ESS again. ESS takes a single player of a population (let's call player $1$) and looks at the interaction of player $1$ with another member of the population with the knowledge that every member of this population (except for player $1$ that we are looking at) plays strategy $s$ with probability $1-\epsilon$.
 %
 Since both players are drawn from the same population, there is an inherent symmetry in the payoffs; therefore, if we show that player $1$ follows the strategy $s$, every other player of this population will also play strategy $s$ in their next interaction.
 %

 Here, there are $N$ players, and all of them interact simultaneously, contrasting to the concept of ESS in which only two players interact. 
%  %
%  Moreover, since here players have different {\power}s their payoffs might not be symmetric. However, we can adopt the concept of ESS and define \textit{reformed ESS} as follow:

%  \begin{definition}(reformed ESS)\label{def:reformed-ESS}
%      In the game $\Gamma_0$ with players $\N = \{1,2,\dots,N\}$ and with the player $i$'s payoff function $u_i(.)$ described in the table \ref{tabular:game0}, strategy $\Ph$ is a reformed ESS strategy if $\forall i \in \N$ there exists $\hat{\epsilon}>0$ such that :
%      $$\epsilon u_i(\Ph,\Vh < \threshold) + (1-\epsilon)u_i(\Ph,\Vh \geq \threshold) > \epsilon u_i(\Pm,\Vh < \threshold) + (1-\epsilon)u_i(\Pm,\Vh \geq \threshold)$$
%  \end{definition}

%  We can interpret the definition of the reformed ESS as similar to ESS. If there is a small possibility $\epsilon < \hat{\epsilon}$ that other players deviate from $\Ph$ and cause $\Vh < t$, every single player of the game still strictly benefits from playing $\Ph$. 
% %

%  Having the definition of reformed ESS we can immediately prove the following theorem. The proof is almost the same as the proof of theorem \ref{theorem:ESS} but it is eliminated due to lack of space.
 
% \begin{theorem}\label{theorem:refined-ESS}
%     Strategy $\Ph$ in the game $\Gamma_0$ is a reformed ESS if and only if $\forall I \in \N$ one of the two conditions obtains:
%     \begin{itemize}
%         \item $u_i(\Ph,\Vh \geq \threshold)>u_i(\Pm,\Vh \geq \threshold)$
%         \item $u_i(\Ph,\Vh \geq \threshold)=u_i(\Pm,\Vh \geq \threshold)$ and $u_i(\Ph,\Vh < \threshold)>u_i(\Pm,\Vh < \threshold)$
%     \end{itemize}
% \end{theorem}

%  We can easily verify that since $\Rdi < \Rhi$, the first condition of the theorem  \ref{theorem:refined-ESS} holds, $\Ph$ is a reformed ESS.
% %
%  This implies that even if $i$ knows that with a small probability $\epsilon \in (0,\hat{\epsilon})$ $\Pm$ becomes the dominant protocol of \Sys, $i$ still prefers to play $\Ph$. 
%  %
%  Since this argument is correct for \textbf{any} player, a small deviation by some nodes would not be followed by others and $\Ph$ is a stable operating point for the system in the absence of any external factor.

 
 \begin{table}\label{table:games}
 \centering
\subfloat[][]{\label{tabular:game0}
 \centering
    \begin{tabular}{p{1.3cm} p{0.7cm}| p{1cm}| p{1cm}| p{0.5cm}} 
       \multicolumn{5}{c}{\hspace{1cm} others}  \\
       & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\Vh \geq \threshold$}  & \multicolumn{1}{c}{$\Vh < \threshold$} &  \\
      \cline{3-4}
      \multirow{2}*{Node $i$}  & $\Ph$ & $\Rhi$ & $\Rdpi$ & \\
      \cline{3-4}
      & $\Pm$ & ${\color{red}\Rdi}$  & $\Rmi$ & \\
       \cline{3-4}\\
    \end{tabular}}
     \qquad
   \subfloat[][]{\label{tabular:game1}
    \centering
    \begin{tabular}{p{1.3cm} p{0.7cm}| p{1cm}| p{1cm}| p{0.5cm}}
       \multicolumn{5}{c}{\hspace{1cm}  others}  \\
      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\Vm < \threshold$}  & \multicolumn{1}{c}{$\Vm \geq \threshold$} & \\
      \cline{3-4}
      \multirow{2}*{Node $i$}  & $\Ph$ & $\Rhi$ & $\Rdpi$ & \\
      \cline{3-4}
      & $\Pbsc$ & ${\color{Green}\Rhi}$  & $\Rmi$ & \\
       \cline{3-4}\\
    \end{tabular}
    }
    \caption{games\zhq{missing description.}}
\end{table}


\subsection{Game 1: Magnate-Coordinated Collusion}\label{subsec:game1}
Table \ref{tabular:game1} demonstrates the utility of an arbitrary player $i$ when playing with a virtual player that determines $\Vh$. In this game contrasting to the game \ref{tabular:game0}, $\Ph$ is not an ESS and we prove that $\Pm$ is the only ESS of this game. 

\begin{theorem}\label{theorem:game1}
     In the game represented in table \ref{tabular:game1}, if $\Rdpi < \Rhi$ then $M'$ is the unique ESS.
 \end{theorem}
 \begin{proof}
  The first condition of the theorem \ref{theorem:ESS} holds for $M$ however none of the conditions stated in he theorem \ref{theorem:ESS} holds for $H$ therefore $M'$ is the unique ESS of the game. 
 \end{proof}

 Theorem \ref{tabular:game1} implies that in the presence of the \bsc, when \Sys starts from its healthy operating point $\Ph$, even an infinitesimal possibility of deviating to $M'$ (following the \bsc) by enough nodes, would incentives all the players to deviate to $M'$. And since $M'$ is an ESS, it is a stable point and the system remains there even with the possibility of deviation of other nodes to $\Ph$.


Our results implies that even in a healthy system in which everybody plays the honest protocol if some nodes deviate even with an infinitesimal probability, the rest would also deviate to following the \bsc. 
%
 In short, factors outside of \Sys can deviate the expected behavior of rational \cns maintaining \Sys. 

%


%








==> draft/formal_model.tex <==
\section{Game theoretic analysis}
In this section, we formalize the current situation of a permissionless blockchain in a game theoretic setting, then we show how, in the presence of the smart contract described in section \ref{} the game changes. And finally, we show that in the presence of such a smart contract, a rational party would never play the honest protocol $\ph$,  and therefore, we defeat the blockchain.

\subsection{Game 1 : In the absence of the \smartContract}
There is a set of rational players $\mathcal{N}=\{1,2,\dots,N\}$ actively working on a blockchain \block. Each player $i$ has hashing power $H_i$ and chooses to consume this hashing power on protocol $\ph$ (honest protocol) or $\pmal$ (malicious protocol). The overall hashing power of all the players is denoted by $\HPowertot$.
%
$\ph$ is a protocol that is designed to be the operating point of the blockchain, and honest players are supposed to follow it. However, there is another protocol,$\pmal$, that, if played by the majority of the hashing power, would disrupt the normal behavior of the blockchain \block and overtake it. 

Now we formally define our first strategic form game $\Gamma_1 = (\mathcal{N} , \{\ph , \pmal\}^N , ({reward}_i)_{i \in \mathcal{N}})$. The set of pure strategies for each player is $\{\ph , \pmal\}$, and we denote the chosen strategy of player $i$ by $s_i$. Here we only consider pure strategies because later, we prove that a rational player would never play a mixed strategy which means that player either follow protocol $\ph$ or $\pmal$. We define two functions $\HPowerh(\mathbf{s})$ and $\HPowermal(\mathbf{s})$ as follow :

$$\HPowerh(\mathbf{s}) := \sum_{j|s_j=\ph} H_j , \quad \HPowermal(\mathbf{s}) := \sum_{j|s_j=\pmal} H_j $$
 
Now we are ready to define the utility function of $\Gamma_1$.
$reward_i$ is a function of the strategy vector $\mathbf{s} = (s_1,\dots,s_N)$ and is defined as follows:

 \[
    reward_i =
  \begin{cases}
        \frac{H_i}{\HPowerh} & \text{If } s_i= \ph \text{ and } \HPowerh > \HPowermal\\
        0 & \text{If } s_i= \ph \text{ and } \HPowerh < \HPowermal\\
        \frac{H_i}{\HPowermal} & \text{If } s_i= \pmal \text{ and } \HPowerh < \HPowermal\\
        0 & \text{If } s_i= \pmal \text{ and } \HPowerh > \HPowermal\\
        \end{cases}
  \]

This reward function, in summary, means that if a player is playing the same protocol as the majority of the hashing power, then it can earn a reward proportional to its hashing rate. Otherwise, it earns nothing. In $\Gamma_1$ as long as no party possesses half or more than half of the hashing power, $\ph$ is a strict Nash Equilibrium. All the existing blockchains are working based on this fact. However, in the following, we show how the existence of the {\smartContract} changes the game.

\subsection{Game 2 : When {\smartContract} exists}
{\smartContract} works as follows:
\begin{enumerate}
    \item \smartContract is deployed. Players can join the smart contract before the predetermined time $T_{join}$ 
    \item Players $i$ willing to join the smart contract announces a hash function of its hashing power $Sha256(H_i)$ and waits until $T_{join}$ passes.
    \item After $T_{join}$ all the players reveal their hashing power $H_i$; it should correspond to the committed value $Sha256(H_i)$ otherwise the smart contract identifies it and doesn't recognize the player as a legitimate player.
    \item smart contract calculates the overall hashing power committed by legitimate players to the smart contract denoted by $\HPowersc$; if $\HPowersc < \frac{HPowertot}{2}$ the attack is aborted and the smart contract life cycle ends otherwise if $\HPowersc > \frac{HPowertot}{2}$ then smart contract announces that the attack should be launched.
    \item After this announcement, legitimate players deposit $d_i$ into the smart contract. We will explain later how $d_i$ should be determined based on $H_i$.
    \item legitimate players should start running the protocol $\pmal$ before a predetermined time  $T_{end}$.  
    \item At time $T_{end}$, the smart contract fetches the activity report of players from an oracle and determines whether the attack was successful, i.e., whether the majority of the hashing power ran $\pmal$ in reality. If the attack were successful, the players who ran $\pmal$ with the correct hashing power withdraw their deposit, they would also earn a profit from the \smartContarct; 
    %in addition to the implicit natural reward of working on $\pmal$ with the majority. 
    However, the players whose activity report doesn't match their commitment lose their deposit and don't earn any profit.
    \item On the other hand, if the attack was unsuccessful, this means that some of the players who committed to run $\pmal$ didn't run it in reality, those players would be identified based on their activity report, and their deposit would be burnt. The rest of the players can withdraw their deposit however they don't earn any profit.
\end{enumerate}


% Now we formally define the strategic form game when {\smartContract} is deployed. $\Gamma_2 = (\mathcal{N} , \{\sh, \scommit , \scheat\}^N , ({reward}_i)_{i \in \mathcal{N}})$. The set of pure strategies for each player is $\{\sh, \scommit , \scheat\}$ where $\sh$ is following the honest strategy $\ph$, $\scommit$ is committing to 




% Here we only consider pure strategies because later, we prove that a rational player would never play a mixed strategy which means that player either follow protocol $\ph$ or $\pmal$. We define two functions $\HPowerh(\mathbf{s})$ and $\HPowermal(\mathbf{s})$ as follow :

% $$\HPowerh(\mathbf{s}) := \sum_{j|s_j=\ph} H_j , \quad \HPowermal(\mathbf{s}) := \sum_{j|s_j=\pmal} H_j $$
 
% Now we are ready to define the utility function of $\Gamma_1$.
% $reward_i$ is a function of the strategy vector $\mathbf{s} = (s_1,\dots,s_N)$ and is defined as follows:

==> tables/table_1.tex <==
\begin{table}\centering
    \setlength{\extrarowheight}{2pt}
    \begin{tabular}{cc|c|c|}
      & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Player $2$}\\
      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\ph$}  & \multicolumn{1}{c}{$\pmal$} \\\cline{3-4}
      \multirow{2}*{Player $1$}  & $\ph$ & $( \frac{H_1}{H_1+H_2},\frac{H_2}{H_1+H_2})$ & $(1,0)$ \\\cline{3-4}
      & $\pmal$ & $(1,0)$ & $\frac{H_1}{H_1+H_2},\frac{H_2}{H_1+H_2})$ \\\cline{3-4}
    \end{tabular}
  \end{table}
